Efectos del campo magn\'etico en un gas de bosones vectoriales neutros: aplicaciones astrof\'isicas

In this thesis, the effects of the magnetic field on neutron stars matter are studied, assuming that the neutrons inside these stars are partially or totally paired forming neutral vector bosons. The main effects of the magnetic field on the gas are, first, to favor the phase transition to the Bose-Eintein condensation, and second, to split the pressure in two components, one parallel and the other perpendicular to the magnetic axis, giving rise to anisotropic equations of state. At low densities or high magnetic fields, the lowest pressure can be negative, and the boson system becomes susceptible to suffer a transverse magnetic collapse. On the other hand, when the temperature is low enough, the gas can spontaneously magnetize. The equations of state of the magnetized gas of neutral vector bosons are applied, firstly, to study the magnetic collpase of an ideal gas of neutrons, electrons and protons (npe gas) in which the nucleons are partially bosonized. From the results obtained, a model for the ejection of matter out of the star and the formation of astrophysical jets is proposed. Subsequently, the equations of state of the magnetized vector gas are used to study the magnetic field influence on the structure (mass, radius and deformation) of Bose-Einsten condensate stars, that is, of compact objects composed entirely by a neutron gas fully bosonized. In order to appropriately take into account the magnetic anisotropy in the equations of state of this object, we develope a system of equations to describe the hydrodynamic equilibrium -- the structure -- of spheroidal compact objects starting from an axisymmetric metric. The obtained results validate the bosons self-magnetization as a feasible source for the magnetic field of compact objects.

==> appF.tex <==
\chapter{Ecuaciones de estado para Enanas Blancas magnetizadas}
\label{appF}

Typical WDs are composed by carbon or oxygen atoms. The role of the different particles conforming these atoms in the star's physics depends on their masses. Due to its relative low mass, only the degenerated gas of relativistic electrons determine the pressure that compensates the gravitational collapse of the star. The heavier neutrons and protons behave non-relativistically, and contribute mainly to the mass and energy density.

The pressures and the energy density of the electron gas in magnetized WDs are obtained starting from the thermodynamical potential \cite{2000PhRvL..84.5261C} \footnote{All expressions in this Section are in natural units, where $\hbar=c=1$.}:
%
\begin{equation}\label{Thermo-Potential}
\Omega(B,\mu,T)=-\frac{e B}{2\pi^2}\int_{0}^\infty dp_3\sum_{l=0}^{\infty}g_l \bigg[ \varepsilon_l
+T\ln \left(1+e^{-(\varepsilon_l-\mu)/T}\right)\left(1+e^{-(\varepsilon_l+\mu)/T}\right)\bigg],
\end{equation}
%
being $\varepsilon_l=\sqrt{p_3^2+2|eB|l+m^2}$ the electron spectrum in a magnetic field. In Eq.~(\ref{Thermo-Potential}) the magnetic field ${\bf B}$  is supposed uniform, constant and in the $z$ direction, $l$ stands for the Landau levels and the factor $g_l=2-\delta_{l0}$ includes the spin degeneracy of the fermions for $l\neq0$. $T$ is the  absolute temperature, $\mu$ the chemical potential, $m$ is the electron mass and $e$ its charge.

Note that, in general, the thermodynamical potential on Eq.~(\ref{Thermo-Potential}) can be divided in two contributions
\begin{equation}\label{Thermo-Potential-2}
\Omega (B,\mu,T)=\Omega^\text{vac}(B)+\Omega^\text{st}(B,\mu,T).
\end{equation}

The second term, $\Omega^\text{st}(B,\mu,T)$, arises from statistical considerations and reads
%
\begin{equation}\label{Thermo-Potential-st}
\Omega^\text{st}(B,\mu,T)=-\frac{e B}{2\pi^2}\int_{0}^\infty dp_3\sum_{l=0}^{\infty}g_l \bigg[T\ln \left(1+e^{-(\varepsilon_l-\mu)/T}\right)\left(1+e^{-(\varepsilon_l+\mu)/T}\right)\bigg].
\end{equation}
%

When studying WDs, since the surface temperatures detected are much smaller than the Fermi temperature, it is accepted to consider the degenerate limit for the fermion gas ($T\to 0$) to compute the thermodynamical potential \cite{shapiro,camenzind}. In that case, the statistical term becomes
%
\begin{equation}\label{Thermo-Potential-st1}
\Omega^\text{st}(B,\mu,0) = -\frac{eB}{2\pi^2}\int_{0}^\infty \!\!\!\!dp_3\sum_{l=0}^{\infty}g_l(\mu-\varepsilon_l)\Theta(\mu-\varepsilon_l),
\end{equation}
%
where $\Theta(\zeta)$ is the unit step function. From the expression (\ref{Thermo-Potential-st1}), we obtain
%
\begin{equation}\label{Thermo-Potential-Sest}
\Omega^\text{st} (B,\mu,0)= \frac{m^2}{4\pi^2}\frac{B}{B_c}\!\sum_{l=0}^{l_{max}}g_{l}\!\left[ \mu\,p_F -\varepsilon_l^2\ln\!\left(\frac{\mu+ p_F}{\varepsilon_l}\right)\right]\!,
\end{equation}
%
where $l_{max}= I[\frac{\mu^2-m^2}{2eB}]$, $I[z]$ denotes the integer part of $z$ and the Fermi momentum is ${p_F}=\sqrt{{\mu}^2-\varepsilon_l^2}$.

On the other hand, the term $\Omega^\text{vac}(B)$ in Eq.~(\ref{Thermo-Potential-2}):
%
\begin{equation}\label{Thermo-Potential-vac}
\Omega^\text{vac}(B)=-\frac{e B}{2\pi^2}\int_{0}^\infty dp_3\sum_{l=0}^{\infty}g_l \varepsilon_l,
\end{equation}
%
does not depend on the chemical potential nor on the temperature and corresponds to the vacuum. This contribution presents an ultraviolet divergence that must be renormalized \cite{1951PhRv...82..664S}. Depending on the  value of $B$ with respect to the critical magnetic field for electrons, $B_c=m^2/e = 4.4\times10^{13}$~G (Schwinger field)\footnote{The magnetic field at which the cyclotron energy of the electrons is comparable to its rest mass.}, the renormalization of $\Omega^\text{vac}$ leads to one of the following expressions corresponding to the weak $(B<B_c)$ and strong magnetic field ($B>B_c$) limits \cite{2015PhRvD..91h5041F}
%
\begin{subequations}\label{Thermo-Potential-vac1}
	\begin{eqnarray}
	\Omega^\text{vac}_w (B,0,0) &= -\frac{m^4}{90 (2\pi)^2}  \left(\frac{B}{B_c}\right)^{\!4}\!, & \quad B<B_c \\ \label{Thermo-Potential-Svac}
	\Omega^\text{vac}_s (B,0,0) &= \frac{(eB)^2}{24\pi^2(\hbar c)^3}\ln\frac{eB}{m^2}, & \quad B>B_c.
	\end{eqnarray}
\end{subequations}

As pointed out previously, the maximum magnetic field estimated for WDs interiors is around $10^{13}~$G, a value that is of the same order of $B_c$. In astrophysical scenarios the energy scales are determined by the temperature and the density. Then, for WDs in the zero temperature limit, the parameter that will set the relative relevance of magnetic field effects on the system is the density. If we consider typical values of densities for WDs and magnetic fields in weak regime, the system is characterized by the relation $eB \ll m^2 \ll \mu^2$. In this case, the vacuum contribution in Eq.~(\ref{Thermo-Potential-vac1}) can be neglected when compared to the statistical one in Eq.~(\ref{Thermo-Potential-Sest}). Therefore, the thermodynamical potential of the electron degenerate system can be approximated to $\Omega(B,\mu,0) = \Omega^\text{st}(B,\mu,0)$ when working below the Schwinger magnetic field.

In this regime, the distance between Landau levels \mbox{$(\sim eB)$} is small and we can consider the discrete spectrum as a continuum. This allows us to replace the sum over $l$ in Eq.~(\ref{Thermo-Potential-Sest}) by an integral through the Euler-MacLaurin formula \cite{1972hmfw.book.....A}
%
\begin{multline}
\label{eq:EMcL}
\frac{eB}{2} \sum_{l=0}^\infty g_l f(2eBl) \approx eB\!  \int_0^\infty \!\!\! f(2eBl)dl+ \frac{eB}{2}f(\infty) \\
+ \sum_{k=1}^\infty \frac{2^{2k-1} }{(2k)!} (eB)^{2k} B_{2k} \left[f^{2k-1}(\infty)-f^{2k-1}(0)\right],
\end{multline}
%
where $f(2eBl) = (\mu-\varepsilon_l)\Theta(\mu-\varepsilon_l)$ and the coefficients $B_n$ stand for the Bernoulli numbers ($B_2=1/6$). Then, we can expand Eq.~(\ref{Thermo-Potential-st1}) onto the second power on $eB$, and take the classical limit by means of the change of variables $p_\perp^2= 2eBl=p_x^2+p_y^2$, with $p_\perp dp_\perp =eBdl$ \cite{1968PhRv..173.1210C}. Hence, we get the statistical part of the thermodynamical potential as follows
%
\begin{multline}\label{Thermo-Potential-st2}
\Omega^{st}(B,\mu,0) = - \frac{m^4}{12\pi^2} \left[\frac{\mu \sqrt{\mu^2-m^2}}{m^2}\left(\frac{\mu^2}{m^2}-\frac{5}{2}\right)\right. + \frac{3}{2} \ln\left(\frac{\mu+\sqrt{\mu^2-m^2}}{m}\right)
\\
\left.
+ \left( \frac{B}{B_c} \right)^{2} \ln \left(\frac{\mu+\sqrt{\mu^2-m^2}}{m} \right) \right].
\end{multline}
%
From Eq.~(\ref{Thermo-Potential-st2}) we note that, in the weak magnetic field limit, the statistical part of the thermodynamical potential is expressed as a sum of two non-magnetic terms at $\mu \neq 0$ and $T=0$, plus a third term that depends also on the magnetic field.

Matter inside compact stars must be in stellar equilibrium. So, we must impose charge neutrality and baryon number conservation to the energy density and the pressures. With these considerations, the magnetized WDs EoS ---the pressures as a parametric function of the energy density--- becomes
%
\begin{subequations}\label{EoSEB}
	\begin{align}
	E &= \Omega + \mu N +m_N\frac{A}{Z}N  +\frac{B^2}{8\pi},\label{EoS1}\\
	P_{\parallel} &= -\Omega-\frac{B^2}{8\pi}, \label{EoS2}\\
	P_{\perp} &= -\Omega-B\mathcal{M}+\frac{B^2}{8\pi},\label{EoS3}
	\end{align}
\end{subequations}
%
where $N=-\partial\Omega/\partial\mu$ is the electron particle density and $\mathcal{M}=-\partial\Omega/\partial B$ the magnetization. Here, the thermodynamical potential $\Omega$ is given by Eq.~(\ref{Thermo-Potential-2}), with $\Omega^\text{vac}$  as in Eq.~(\ref{Thermo-Potential-vac1}) and $\Omega^\text{st}$ from Eq.~(\ref{Thermo-Potential-Sest}) or Eq.~(\ref{Thermo-Potential-st2}) according to the value of B. The term $ N m_N A/Z$ included in Eq.~(\ref{EoS1}) considers the contribution of the nucleons to the energy density\footnote{$m_N = 931.494$ MeV $\sim m_{n,p}$ and $A/Z$ is the number of nucleons per electron ($A/Z=2$ for carbon/oxygen WDs)}.

The last term in Eqs.~(\ref{EoSEB}) is the Maxwell contribution to the pressures and energy density, $P_{\perp}^B=E^B=-P_{\parallel}^B=B^2/8\pi$. Contrary to the case of Neutron Stars and Quark Stars \cite{Lattimer}, where the energy density and pressures are of the same order, WDs energy densities are three orders higher than the pressures. Therefore, the value delimiting when the Maxwell term becomes relevant is determined by the pressure, with $P_{\perp}^B$ comparable to the statistical pressures for magnetic fields higher than $1.78\times10^{11}$~G.\footnote{The magnetic energy density becomes relevant at $10^{14}~$G \cite{Terrero:2017mxc}.}

Anyhow, we explore the parametric EoS given in Eqs.~(\ref{EoSEB}) and tackle two cases, the first one neglecting the Maxwell contribution (upper panel of Fig.~\ref{fig:EOS}) and the second one considering it (lower panel), for magnetized WDs with a carbon/oxygen composition at $B=0$, $B=10^{12}$~G, $B=10^{13}$~G and $B=10^{14}$~G. Note that at higher densities there is no appreciable difference between the perpendicular and the parallel pressures while at low densities the anisotropy starts to be noticeable, being the perpendicular pressure curve softer (harder) than the parallel one in the case without (with) Maxwell term.
%
\begin{figure}[!ht]
	\includegraphics[width=0.48\textwidth]{eos}
	\caption{EoS for magnetized WDs at fixed values of the magnetic field for  $B=0$, $B=10^{12}$~G, $B=10^{13}$~G and $B=10^{14}$~G (in CGS units). In the upper panel Maxwell term is neglected while in the lower panel it is considered.}	\label{fig:EOS}
\end{figure}

